Mapping Wireless Networks into Digital Reality through Joint Vertical and Horizontal Learning

In recent years, the complexity of 5G and beyond wireless networks has escalated, prompting a need for innovative frameworks to facilitate flexible management and efficient deployment. The concept of digital twins (DTs) has emerged as a solution to enable real-time monitoring, predictive configurations, and decision-making processes. While existing works primarily focus on leveraging DTs to optimize wireless networks, a detailed mapping methodology for creating virtual representations of network infrastructure and properties is still lacking. In this context, we introduce VH-Twin, a novel time-series data-driven framework that effectively maps wireless networks into digital reality. VH-Twin distinguishes itself through complementary vertical twinning (V-twinning) and horizontal twinning (H-twinning) stages, followed by a periodic clustering mechanism used to virtualize network regions based on their distinct geological and wireless characteristics. Specifically, V-twinning exploits distributed learning techniques to initialize a global twin model collaboratively from virtualized network clusters. H-twinning, on the other hand, is implemented with an asynchronous mapping scheme that dynamically updates twin models in response to network or environmental changes. Leveraging real-world wireless traffic data within a cellular wireless network, comprehensive experiments are conducted to verify that VH-Twin can effectively construct, deploy, and maintain network DTs. Parametric analysis also offers insights into how to strike a balance between twinning efficiency and model accuracy at scale.

==> method.tex <==
\section{System Design} 
\label{sec:system_design}

To address the aforementioned challenges, we introduce an innovative framework termed VH-Twinning, which stands for Vertical and Horizontal Twinning.
This framework is structured around three principal stages: Dynamic Connectivity Segmentation (DCS), Vertical Twinning (V-twinning), and Horizontal Twinning (H-twinning). 
DCS is employed periodically to ensure effective clustering, V-twinning is performed at the beginning to initialize a concrete Global Digital Network Twin (G-DNT), and H-twinning is performed later to update the twins regularly.

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.33]{figs/VH-Twin.pdf}
    \caption{Framework}
    \label{fig:framework}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.5]{figs/SFL.pdf}
    \caption{SFL and AFL}
    \label{fig:framework}
\end{figure}

\subsection{Dynamic Connectivity Segmentation}
% 1. cluster-level digital network twins (C-DNT) are deplyed on each cluster
% 2. DCS algorithm runs periodically to ensure precise clustering
% 3. Proper clustering results in better model performance.
% 4. Clusters are based on geological distance, link strength, coverage area, and distribution similarity in our case, but can be extend to other attributes, such as functionality.
% 5. Girvan Newman Community detection method is used to cluster BSs after knowing the relationships between BSs.
% 6. Models from local BSs are shared to corresponding C-DNT for further updates.

\begin{algorithm}[t]
\caption{Dynamic Connectivity Segmentation (DCS)}
\begin{algorithmic}[1]
\Require relationship matrix \( \{ g, k, \beta, \theta \} \), attribute weights \( \omega \), \( C \) clusters, \( M \) BSs
\Ensure Clusters \( c \)
\State \( \Phi = [] \)
\For{\( m_1 = 1, 2, \ldots, M \)}
    \For{\( m_2 = 1, 2, \ldots, M \)}
        \State \( \Phi_{m_1,m_2} \gets \frac{\omega[0]}{g_{m_1,m_2}} + \frac{\omega[1]}{k_{m_1,m_2}} + \frac{\omega[2]}{\beta_{m_1,m_2}} + \frac{\omega[3]}{\theta_{m_1,m_2}}\)
    \EndFor
\While{desired \( C \) clusters not reached}
    \State Calculate edge connectivity for all edges in \( \Phi \)
    \State Remove edge with the highest connectivity
    \State Recalculate the communities
\EndWhile
\EndFor
\State \Return \( c \)
\end{algorithmic}
\label{algo:DCS}
\end{algorithm}

The Dynamic Connectivity Segmentation (DCS) algorithm, as shown in Algorithm~\ref{algo:DCS}, is integral to the creation and updates of Cluster Digital Network Twins (C-DNT), which are deployed in each cluster. 
This algorithm is executed periodically, ensuring precise clustering and thereby enhancing model performance. 
% 
In the DCS algorithm, clusters are based on an attribute sequence \( \{ g, k, \beta, \theta \} \), which represents geological distance, link strength, coverage area, and distribution similarity, respectively. 
It can be further extended to other attributes like BS functionality. 
Initially, a relationship matrix incorporating these attributes, weighted by \( \omega \), is constructed. 
For each BS \( m_1 \) and BS \( m_2 \) within \(  M  \), the algorithm calculates a metric \( \Phi_{m_1,m_2} \) to represent their relationships using the formula as follows:
\begin{equation}
    \Phi_{m_1,m_2} = \frac{\omega[0]}{g_{m_1,m_2}} + \frac{\omega[1]}{k_{m_1,m_2}} + \frac{\omega[2]}{\beta_{m_1,m_2}} + \frac{\omega[3]}{\theta_{m_1,m_2}}.
\end{equation}
The algorithm clusters BSs by iteratively removing edges with the highest connectivity from \( \Phi \) until the desired number of clusters \( C \) is reached, which is similar to the Girvan-Newman method~\cite{Newman_2004}. 
% 
This clustering process is pivotal in determining how models from local BSs are shared with their corresponding C-DNT for further updates and improvements, and thus update the global digital network twins (G-DNT).

% \( \{ g, k, \beta, \theta \} \), geological distance, link strength, coverage area, distribution similarity

\subsection{Vertical Twinning (V-Twin)}


\begin{algorithm}[t]
\caption{Vertical Twinning (V-Twin)}
\begin{algorithmic}[1]
\Require Local models \( \bm{\alpha}_1^t, \bm{\alpha}_2^t, \ldots, \bm{\alpha}_{M}^t \), \( C \) clusters
\Ensure Updated G-DNT \( \bm{\alpha}^{t+1} \)
\For{\( c = 1, 2, \ldots, C \)}
    \State \( P \gets \text{BS count in cluster } c \)
    \State \(\bm{\alpha}_c^{t} \gets \frac{1}{P}\sum_{p=1}^P \bm{\alpha}_p^{t} \)
\EndFor
\State \( \bm{\alpha}^{t+1} \gets \frac{1}{C}\sum_{c=1}^C \bm{\alpha}_c^{t}\)
\State \Return \( \bm{\alpha}^{t+1} \)
\end{algorithmic}
\label{algo:VT}
\end{algorithm}

% 1. We use federated learning technique to distributed computational load to local BSs and protect data privacy.
% 2. In this stage, FL use historical data to train the cluster-level digital network twin (C_DNT)
% 3. Multi-level FL is used based on clusters because of efficient resource management, energy efficiency, and load balancing
% 4. Synchronous FL is used in this stage for better consistency and stability, and efficient convergence


The Vertical Twinning (V-Twin) stage, as depicted in Algorithm~\ref{algo:VT}, represents an innovative FL strategy, specifically engineered for wireless networks with multiple BSs and clusters. This approach efficiently distributes computational tasks across BSs while ensuring data privacy.

At the core of V-Twin is the use of historical data from each BS \( m \) to train Cluster Digital Network Twins (C-DNTs) for each cluster (\( c \)). A key aspect of V-Twin is aggregating local model updates, denoted as \(\bm{\alpha}_1^t, \bm{\alpha}_2^t, \ldots, \bm{\alpha}_M^t\), from each BS within a cluster. These are merged to form a consolidated C-DNT (\(\bm{\alpha}_c^t\)) for each cluster.
V-Twin employs synchronous FL (SFL), ensuring all clusters update their models simultaneously. This synchronization is crucial for consistent and stable learning processes across the network, leading to effective convergence.
SFL has distinct advantages, particularly in terms of consistency and model convergence. Synchronizing the model updates from all participating clients at regular intervals, ensures a more uniform and controlled learning process, leading to potentially more stable and predictable model performance. Additionally, synchronous FL can simplify the management of updates and reduce issues related to stale or incompatible data, making it suitable for scenarios where uniformity and coordination among clients are critical.

The Global-Digital Network Twin (G-DNT), represented as \(\bm{\alpha}^{t+1}\), is computed by averaging C-DNTs simutaneously as well:
\begin{equation}
    \bm{\alpha}^{t+1} = \frac{1}{C}\sum_{c=1}^C \bm{\alpha}_c^t,
\end{equation}
where \(C\) is the number of clusters. This methodology offers benefits in resource allocation, energy conservation, and load balancing across the network.



\subsection{Horizontal Twinning (H-Twin)}

\begin{algorithm}[t]
\caption{Horizontal Twinning (H-Twin)}
\begin{algorithmic}[1]
\Require Local models \( \bm{\alpha}_1^t, \bm{\alpha}_2^t, \ldots, \bm{\alpha}_{M}^t \), current G-DNT \( \bm{\alpha}^{t} \), \( C \) clusters, threshold \( \eta \)
\Ensure Updated G-DNT \( \bm{\alpha}^{t+1} \)
\For{\( c = 1, 2, \ldots, C \textbf{ asynchronously}\)}
    \State \( P \gets \text{BS count in cluster } c \)
    \State \(\bm{\alpha}_c^{t} \gets \frac{1}{P}\sum_{p=1}^P \bm{\alpha}_p^{t} \)
    \State \( \epsilon \gets (\bm{\alpha}_c^{t} + \bm{\alpha}^{t})^2 \)
    \If{\( \epsilon > \eta \)}
        % \State \text{Share C-DNT to G-DNT}
        \State \( \bm{\alpha}^{t+1} \gets \frac{1}{C}\sum_{c=1}^C \bm{\alpha}_c^{t}\)
    \Else
        % \State \text{Do not share C-DNT to G-DNT}
        \State \( \bm{\alpha}^{t+1} \gets \bm{\alpha}^{t}\)
    \EndIf
\EndFor
% \State \( \bm{\alpha}^{t+1} \gets \frac{1}{C}\sum_{c=1}^C \bm{\alpha}_c^{t}\)
\State \Return \( \bm{\alpha}^{t+1} \)
\end{algorithmic}
\label{algo:HT}
\end{algorithm}


% Similar overall structure is used compared to V-Twin
% Threshold \eta, which measures the difference between current global twin and local twin, is used for infrequent updates
% Asynchronous FL is used due to scalability, reduced communication overhead, and flexibility.

Horizontal Twinning (H-Twin) adopts an Asynchronous Federated Learning (AFL) approach to update with real-time data from physical twins, providing a scalable and flexible solution for wireless networks composed of multiple clusters.
Unlike V-Twin, H-Twin does not require simultaneous updates from all clusters, although the overall structure to compute C-DNT and G-DNT is quite similar. Each BS \( m \) stores the real-time data first, and trains when the amount of data reaches a threshold in batches.
AFL offers several advantages over its synchronous counterpart. Primarily, it allows for greater flexibility in participation, as clients can contribute to the model training process at their own pace and availability, without being bound to a strict synchronization schedule. This feature is particularly beneficial in scenarios with clients having varying computational resources or network connectivity, ensuring that the learning process is inclusive and efficient even in less ideal conditions.

The algorithm begins with local models \(\bm{\alpha}_1^t, \bm{\alpha}_2^t, \ldots, \bm{\alpha}_M^t\) from individual BSs and the current G-DNT \(\bm{\alpha}^t\). A key feature of H-Twin is the use of a threshold \(\eta\), which serves as a criterion to decide whether the G-DNT should be updated.
It computes a C-DNT \(\bm{\alpha}_c^t\) for each cluster \(c\) and then assesses the deviation between this twin and the current G-DNT, quantified by the equation below:
\begin{equation}
    \epsilon = (\bm{\alpha}_c^t + \bm{\alpha}^t)^2.
\end{equation}
If \(\epsilon\) surpasses the threshold \(\eta\), indicating a significant change, the G-DNT is updated to reflect the new information. The updated G-DNT, \(\bm{\alpha}^{t+1}\), is calculated as an average of the cluster-level models, \(\bm{\alpha}^{t+1} = \frac{1}{C}\sum_{c=1}^C \bm{\alpha}_c^t\). If \(\epsilon\) is within the threshold \(\eta\), G-DNT stays with the current model, \(\bm{\alpha}^{t+1} = \bm{\alpha}^t\). This threshold-based update mechanism enhances the network's efficiency by ensuring that only significant changes lead to updates, thereby reducing unnecessary computational overhead and preserving bandwidth.



==> method_backup.tex <==
% !TEX root = mainfile.tex

\section{System Design} 

To address the aforementioned challenges, we introduce an innovative framework termed VH-Twin, which stands for Vertical and Horizontal Twinning.
This framework is structured around three principal stages: clustering, Vertical Twinning (V-Twin), and Horizontal Twinning (H-Twin). 

In the Vertical Twinning phase, all base stations (BSs) collaboratively construct a unified digital twin by utilizing historical data derived from their physical twins. Subsequently, during the Horizontal Twinning phase, these digital twins undergo real-time updates whenever significant disparities are observed between the current and previous models. These updates are based on real-time data garnered from the physical twins. Importantly, VH-Twin employs distributed learning techniques to surmount challenges related to data leakage, data privacy, communication overhead, and computational efficiency in a centralized setting.

\subsection{Vertical Twinning}

% In the vertical twinning stage of our model, federated learning techniques are employed to collaboratively train a global twin. This approach accommodates the unique characteristics of each local base station (BS), such as diverse geological locations, varied data distributions, disparate coverage areas, and different link strengths.

% Due to these heterogeneities, it is essential to group the base stations into multiple clusters to optimize modeling performance. Moreover, it's important to recognize that these base stations could be owned by different enterprises or be designed for specialized purposes. As such, their distinct functionalities should also be factored into the clustering algorithm.
% To achieve effective clustering, we employ a metric called "betweenness" to evaluate the relationships between all pairs of base stations. This metric integrates several key variables: the geographical proximity of the stations, the strength of communication links, and their corresponding coverage areas. Our clustering algorithm iteratively identifies and removes the link with the lowest betweenness score, effectively separating base stations that are less similar according to these criteria.
% After each removal, the betweenness scores are recalculated to reflect the updated network topology. This iterative process continues until satisfies the pre-defined condition. This clustering algorithm should be performed every a few training rounds for better results.

% After effective clustering, a multi-level federated learning architecture is introduced to further refine the performance and generalization of the model. Within each cluster, virtual Base Stations (vBSs) initiate the learning process by collecting historical data from their corresponding physical twins. Utilizing this data, each vBS trains a high-fidelity model that accurately captures the functionality and behavior of its associated physical Base Station (BS).

% Subsequently, these vBSs share their model parameters with a designated local twin for aggregation. This local aggregation serves to generalize the models by combining insights from multiple vBSs, thereby enhancing the overall predictive performance and robustness within the cluster.
% Once a refined local twin is established for each cluster, the next phase involves another aggregation at the global twin level. The global twin aggregates model parameters received from all the local twins, thus synthesizing a comprehensive, unified model that encapsulates the characteristics and insights from all clusters.
% It is crucial for both local and global aggregation processes to be carried out synchronously. Synchronous updates ensure better convergence performance, as they align the model parameters across different twins, allowing for a more consistent and unified model. Furthermore, synchronous updating minimizes the risk of update congestion or conflicts, thereby ensuring that the system remains stable and reliable throughout the learning process.


In the vertical twinning stage of our framework, federated learning methodologies are harnessed to cooperatively cultivate a comprehensive twin model. Each local base station (BS) oversees a subdivision of the traffic data sequence \( \mathcal{D} = \{d_1, d_2, \ldots, d_M\} \). The mission is to calibrate a global loss function \( \mathcal{H} \) across all BSs, recognizing their distinct traits such as geographical placement, data profiles, coverage zones, and connection robustness. Mathematically, the local model for the \( l \)-th BS is articulated as
\begin{equation}
y^l_k = \mathfrak{F}(d_{m-\rho:m}; \boldsymbol{\Theta}^l),
\end{equation}
where \( \mathfrak{F} \) symbolizes the local forecasting function, and \( \boldsymbol{\Theta}^l \) embodies the model parameters for the \( l \)-th BS.

Acknowledging the diversity amongst base stations, it is pivotal to stratify them into consortia with analogous features. These could be under varying proprietorships or engineered for particular functions. To stratify the BSs, we introduce a "betweenness" metric \( \mathcal{B} \) delineated as:
\begin{equation}
\mathcal{B}(i, j) = \mathfrak{F}(\mathcal{G}, \mathcal{W}_{ij}),
\end{equation}
where \( \mathcal{G} \) is the graph depicting network topology, and \( \mathcal{W}_{ij} \) represent the coefficients signifying essential factors such as link robustness and spatial adjacency.

Our clustering paradigm operates recursively, pinpointing and excluding the link with the minimal betweenness valuation, thus efficiently segregating dissimilar BSs. Following each iteration, the betweenness valuations are recalculated to refresh the network graph. This recursive method proceeds until a stipulated criterion is achieved. Periodically reevaluating this clustering is recommended to boost efficacy.

Subsequent to effective stratification, a hierarchical federated learning structure is enacted. Virtual Base Stations (vBSs) within each cluster commence the learning sequence utilizing the historical data subsets \( x^l_k \). They endeavor to curtail the loss function \( \mathcal{H} \), with local parameter increments \( \Delta \boldsymbol{\Theta}^l \) prescribed by:
\begin{equation}
\Delta \boldsymbol{\Theta}^l = -\eta \nabla \mathcal{H}(\mathfrak{F}(x^l_k; \boldsymbol{\Theta}^l), y^l_k),
\end{equation}
where \( \eta \) signifies the learning coefficient.

These vBSs subsequently convey their model parameters \( \boldsymbol{\Theta}^l \) to a nominated local twin for amalgamation. The synthesized local model parameters \( \boldsymbol{\Phi}_{\text{local}} \) are calculated as:
\begin{equation}
\boldsymbol{\Phi}_{\text{local}} = \frac{1}{L} \sum_{l=1}^{L} \boldsymbol{\Theta}^l.
\end{equation}

Ultimately, the global twin integrates these local twins to formulate a consolidated model parameter \( \boldsymbol{\Phi} \) through:
\begin{equation}
\boldsymbol{\Phi} = \frac{1}{N} \sum_{n=1}^{N} \boldsymbol{\Phi}_{\text{local}}^n,
\end{equation}
where \( N \) epitomizes the number of local clusters.

It is imperative that both local and global integration phases are executed in synchrony. This promotes enhanced convergence by normalizing the model parameters across the various echelons of the architecture, concurrently mitigating the potential for update blockages or discrepancies, thereby preserving the system's stability and dependability throughout the learning trajectory.



\subsection{Horizontal Twinning}

% In the horizontal twinning stage, we employ real-time asynchronous updates to ensure a high-fidelity representation of the physical twin in the current global twin model. During this process, an effective clustering strategy enhances the system's trustworthiness. Specifically, clustering improves real-time adaptability by enabling rapid adjustments to fluctuating conditions and data distributions within the wireless network. Additionally, it strengthens security and privacy measures by confining data exchanges to localized clusters, and optimizes fault recovery by streamlining task reallocation among adjacent base stations. To maintain these advantages, the clustering algorithm is periodically revisited and updated.

% The training regimen in the horizontal twinning stage shares similarities with that of the vertical twinning stage but diverges in two crucial aspects. First, asynchronous Federated Learning (FL) is utilized during the sharing of parameters between local and global twins, substantially minimizing waiting time and thus boosting training efficiency. Second, we adopt cosine similarity as a metric to assess the congruence between the local and global twins. Updates to the global twin are triggered only when significant differences arise, as indicated by a cosine similarity score exceeding a pre-defined threshold. This selective updating strategy not only minimizes the frequency of twin synchronizations but also substantially reduces communication overhead. The horizontal twinning stage offers the distinct advantages of scalability and real-time adaptability, making it particularly suited for dynamic and large-scale wireless networks.

In the horizontal twinning stage, real-time asynchronous updates are deployed, denoted as:
\begin{equation}
\tilde{y^l_k} = \mathfrak{G}(d_{m-\rho:m}; \tilde{\boldsymbol{\Theta}}^l),
\end{equation}
where \( \mathfrak{G} \) symbolizes the asynchronous forecasting function and \( \tilde{\boldsymbol{\Theta}}^l \) are the asynchronous model parameters for the \( l \)-th BS. This asynchronous modality substantially diminishes latency and augments the system's scalability. To appraise the congruence between the local and global twins, we deploy a cosine similarity metric \( \mathcal{S} \), defined by:
\begin{equation}
\mathcal{S}(l, \mathcal{G}) = \frac{\boldsymbol{\Theta}^l \cdot \boldsymbol{\Phi}}{\|\boldsymbol{\Theta}^l\|_2 \|\boldsymbol{\Phi}\|_2},
\end{equation}
The global twin undergoes an update exclusively if \( \mathcal{S}(l, \mathcal{G}) \) surpasses a predetermined threshold \( \tau \).
% \begin{equation}
% \text{if } \mathcal{S}(l, \mathcal{G}) > \tau \text{ then update } \boldsymbol{\Phi}.
% \end{equation}
This judicious updating modulates the update frequency, thus diminishing communication burden. The virtues of horizontal twinning are embedded in its scalability and instantaneous adaptability, ensuring that the system can nimbly conform to dynamic scenarios whilst minimizing communication expenditures.

\begin{algorithm}
\caption{VH-Twin Framework}
\begin{algorithmic}[1]
\State \textbf{Initialize:} Preload historical datasets, establish initial model parameters \( \boldsymbol{\Theta}^l \) for each Base Station (BS)

\Comment{Vertical Twinning}
\For{each local BS \( l \)}
    \State Cultivate model \( \mathfrak{F}(d_{m-\rho:m}; \boldsymbol{\Theta}^l) \) with historical data \( x^l_k \)
    \State Deduce local parameter enhancements \( \Delta \boldsymbol{\Theta}^l \)
    \State Dispatch \( \Delta \boldsymbol{\Theta}^l \) to local twin
\EndFor
\State Amalgamate \( \boldsymbol{\Phi}_{\text{local}} = \frac{1}{L} \sum_{l=1}^{L} \boldsymbol{\Theta}^l \)
\State Formulate global twin parameter \( \boldsymbol{\Phi} = \frac{1}{N} \sum_{n=1}^{N} \boldsymbol{\Phi}_{\text{local}}^n \)

\Comment{Horizontal Twinning}
\State \textbf{Reinitialize:} Stream real-time data
\While{streaming real-time datasets}
    \For{each local BS \( l \)}
        \State Execute model training asynchronously
        \State Infer asynchronous local parameter enhancements \( \Delta \boldsymbol{\Theta}^l \)
        \State Relay \( \Delta \boldsymbol{\Theta}^l \) to local twin
        
    \EndFor
    \If{\(\mathcal{S} > \tau\)}
        \State Convey \( \Delta \boldsymbol{\Theta}^l \) to global twin
        \State Merge \( \boldsymbol{\Phi}_{\text{local}} \) asynchronously
        \State Refresh global model parameter \( \boldsymbol{\Phi} \) asynchronously
    \EndIf

\EndWhile
\end{algorithmic}
\end{algorithm}




